Probabilistic Management of OCR Data using an RDBMS

The digitization of scanned forms and documents is changing the data sources that enterprises manage. To integrate these new data sources with enterprise data, the current state-of-the-art approach is to convert the images to ASCII text using optical character recognition (OCR) software and then to store the resulting ASCII text in a relational database. The OCR problem is challenging, and so the output of OCR often contains errors. In turn, queries on the output of OCR may fail to retrieve relevant answers. State-of-the-art OCR programs, e.g., the OCR powering Google Books, use a probabilistic model that captures many alternatives during the OCR process. Only when the results of OCR are stored in the database, do these approaches discard the uncertainty. In this work, we propose to retain the probabilistic models produced by OCR process in a relational database management system. A key technical challenge is that the probabilistic data produced by OCR software is very large (a single book blows up to 2GB from 400kB as ASCII). As a result, a baseline solution that integrates these models with an RDBMS is over 1000x slower versus standard text processing for single table select-project queries. However, many applications may have quality-performance needs that are in between these two extremes of ASCII and the complete model output by the OCR software. Thus, we propose a novel approximation scheme called Staccato that allows a user to trade recall for query performance. Additionally, we provide a formal analysis of our scheme's properties, and describe how we integrate our scheme with standard-RDBMS text indexing.

==> sec_appen.tex <==
%\section{Material for Section~3}

\begin{figure*}[hbtp]
\centering
\includegraphics[width=7in]{images/gadgets}
\caption{Gadgets used in the proof of Theorem 3.1: (A) Overall Reduction. 
We create one block for each of the $N$ sets $\mathcal{S}_i$
(B) Multiply Gadget (C) Binary Exclusive Gadget
}
\label{fig:gadgets}
\vspace{-10pt}
\end{figure*}


\eat{\subsection{Partitioning SFAs is NP-Hard}
\label{app:partition}

Our claim follows by a simple observation in the proof of Shum and
Trotter's proof that a related problem is
hard~\cite{Shum:1996:CCA:230094.230124}. The {\em chain partition
  problem} is given as input a lattice, determine whether it is
possible to decompose the lattice into chains of length $3$. This
problem is \NP-Hard. The first observation is that an SFA of length
$3$ is either a chain or a triangle (since it is a DAG). We observe
that Shum and Trotter's a gadget reduction is triangle free. Thus, any
partition into length $3$ SFAs is also into length $3$ chains. In our
problem, there is no constraint that every chain must be exactly
length $3$. However, it is clear that if we could minimize the number
of SFAs (and so chains), that the original graph of $3N$ nodes admits
an exact decomposition into $3$ chains if and only if the
decomposition that uses the fewest number of chains contains exactly
$N$ chains. Thus, our minimization problem is at least as hard.
}

\fullversion{
\section{Conditional is a $\mathsf{KL}$ Minimizer}
\label{app:kl}

$\mathsf{KL}$ divergence is similar
  to a distance metric in that it allows us to say whether or not two
  probability distributions are close. Given two probability
  distribution $\mu,\nu : \Sigma^{*} \to [0,1]$ the $\KL$-divergence
  is denoted $\KL(\mu || \nu)$ and is defined as:
\[ \KL(\mu || \nu) = \sum_{\sigma \in \Sigma^{*}} \mu(x) \log \frac{\mu(x)}{\nu(x)} \]
The above quantity is only defined for $\mu,\nu$ such that $\mu(x) >
0$ implies that $\nu(x) > 0$. If $\mu = \nu$ then $\KL(\mu || \nu) =
0$.


We justify our choice to retain the probability of each string we
select by showing that it is in fact a minimizer for a common
information theoretic measure, $\mathsf{KL}$-divergence. Given a
probability distribution $\mu$ on $\Sigma^{*}$ and a set $X \subseteq
\Sigma^{*}$, let $\mu_{|X}$ denote the result of conditioning $\mu$ on
$X$. Let $A$ be the set of all distributions on $X$. Then,
\begin{equation}
 \KL( \mu_{|X} || \mu) \leq \min_{\alpha \in A} \KL( \alpha ||
\mu) 
\label{eq:propto}
\end{equation}
That is, selecting the probabilities according to the conditional
probability distribution is optimal with respect to $\KL$
divergence. Eq.~\ref{eq:propto} follows from the observation that
$\KL(\mu_{|X} || \mu) = - \log Z$ where $Z = \sum_{x \in X}
\mu(x)$. Using the log-sum inequality one has
\[ \sum_{x \in X} \alpha(x) \log \frac{\alpha(x)}{\mu(x)} \geq 
\left(\sum_{x \in X} \alpha(x)\right) \log \frac{ \left(\sum_{x \in X}
    \alpha(x) \right)}{ \left(\sum_{x \in X} \mu(x) \right) }
= - \log Z \]
}

\section{$\delta_k$ is a minimizer (Proposition~\protect\ref{prop:min})}

Consider any chunk $(S_i,s,f)$ where $s$ is the single start state and
$f$ is the final state. By constructing, every path that uses a a
character from $S_i$ must enter through $s$ and leave through $f$. And
the higher probability that we place in that state, the higher the
retained mass. Since $\delta_k$ retains the highest probability in
each segment it indeed retains the highest probability mass.


\section{Sketch of Theorem~\protect\ref{THM:HARD}}
 
The starting point is that the following problem is \NP-hard: Given 
vectors $x,y \in \mathbb{Q}^{l}$ and a fixed constant $\lambda \geq 0$
for $l=4$ and sets of stochastic matrices
$\mathcal{S}_1,\dots,\mathcal{S}_N$ where each $\mathcal{S}_i$ is a
set of $2$ $l \times l$ matrices, determine if there is a sequence
$\bar i \in \set{1,2}^{N}$ such that $M_{i_j} \in \mathcal{S}_j$ and:
\[ x^{T} M_{i_N} \cdots M_{i_1} y \geq \lambda \]

We find a small $l$ such that the claim holds. For this, we start with
the results of Bournez and Branicky show that a related problem called
the {\em Matrix Mortality problem} is \NP-hard for matrices of size $2
\times 2$~\cite{DBLP:journals/mst/BournezB02}, where we ask for to
find a selection as above where $x^T M_{i_N} \cdots M_{i_1} y =
0$. Unfortunately, the matrices $(M_{ij})$ are not stochastic (not
even positive). However, using the techniques of Turakainen \cite{turakainen:1969}
 (and Blondel~\cite{DBLP:journals/ipl/BlondelT97}), we can transform the
matrices into slightly larger, but still constant dimensions,
stochastic matrices ($4$ above).

Now, we construct a transducer and chunk $\Phi$
structure such that if it is possible to choose at most $k=2$ in each
chunk with the total probability mass being greater than $\lambda 2^{-N}$, 
then we can get a choice for $\bar i$. Equally, if there exists such a choice 
for $\bar i$, then we can find such a transducer representation.
So the problem of
finding the highest mass representation is \NP-hard as well.

Throughout this reduction, we assume that every edge is assigned a
unique character to ensure the unique path property. In the full
version, we show how to optimize for a binary alphabet. So, we omit
the emitted string in the transition function.


Let $P(x)$ denote the probability mass that a string is emitted that
passes through the node $x$. We will group nodes together as
components of a vector. The start node $s$ has $P(s) = 1$. Then, we
construct the vector $y$ by creating nodes $v_1,\dots,v_l$ with a
transition $\delta((s,v_i), 0) = y_i$. Thus, $P(v_i) = y_i$. We need two
main gadgets: (1) A gadget to encode matrix multiplication and (2) a
gadget that intuitively encodes that given two inputs, we can select
one or the other, but not both. We provide a slightly weaker property:
For a fixed parameter $\alpha \geq 0$ (we pick $\alpha$ below). We
construct a gadget that takes as input two nodes $x, x'$ and has
output two nodes $u, u'$ such that the probability at $u$ ($P(u)$) and
at $u'$ ($P(u')$) satisfies the following property:
\begin{equation}
(P(u),P(u')) = \set{(P(x),0), (0,P(x')), (v,v')} 
\label{eq:exclusive}
\end{equation}
\noindent where $v \leq \alpha P(x)$ and $v' \leq \alpha
P(x')$. Intuitively, this gadget forces us to choose $x$ or $x'$ or
not both. Notice that if we select both, then each component is
smaller than $\alpha$.

Assuming these gadgets, the overall construction is shown in
Figure~\ref{fig:gadgets}(A) that illustrates a chunk for a single set
$\mathcal{S}_i$. Each chunk contains two matrix multiply gadgets
(representing the two matrices in $\mathcal{S}_i$) and a large gadget
that ensures we either choose one matrix or the other -- but not
elements of both.  The input to the chunk is a vector $x$: in the
first chunk, $x = y$ above. In chunk $j$, $x$ will represent the
result of some of choice $M_{i_{j-1}} \cdots M_{i_{1}} y$. As shown,
for each $i=1,\dots,l$, we send $x_i$ to $v_i$ with probability $0.5$
and $x_i$ to $u_i$ with probability $0.5$. In turn, $u$ is fed to the
multiply gadget for $M_{1j}$ and $v$ is fed to the multiply gadget for
$M_{2j}$ (with $\delta$ = 1). We ensure that we cannot select both
$v_i$ and $u_j$ for any $i,j$ using the exclusive gadget described
below. The output of this chunk is either $0.5M_{i1}x$ or $0.5
M_{i2}x$ or a vector with one norm smaller than $\alpha$. We set
$\alpha < 2^{-N}\lambda$. Given any solution to the original problem,
we can create a solution to this problem. On the other hand, if the
solution with highest probability mass has mass greater than $2^{-N}
\lambda$, then it must be a valid solution (since we set $\alpha <
2^{-N}\lambda$). Now the gadgets:


\eat{\begin{figure}
\includegraphics[width=3in]{images/gadgets1}
\caption{Multiply Gadget}
\label{fig:multiply}
\end{figure}
}
\paragraph*{The Multiply Gadget}
Matrix multiplication can be encoded via a transducer (see
Fig.~\ref{fig:gadgets}(B)). Notice that the ``outputs'' in the above
gadget have the probability of the matrix multiply for $2\times 2$
matrices. That is, given a matrix $A$ and input nodes $x_1,\dots,x_m$,
the output nodes $y_i$ above are such that $P(y_i) = \sum_{j=0}^{m}
A_{ij} P(y_j)$. Each edge is one chunk.


\eat{\begin{figure}
\includegraphics[width=3in]{images/gadgets2}
\caption{Binary Exclusive Gadget}
\label{fig:multiply}
\end{figure}
}

\paragraph*{The Exclusive Gadget}
We illustrate the gadget for $k=2$. We have two inputs $x,x'$ and
two outputs $u,u'$. Our goal is to ensure the property described by
Eq.~\ref{eq:exclusive}. The gadget is shown in
Figure~\ref{fig:gadgets}(C). The chunk here contains the entire
gadget, since we can only select $k$ paths, it is clear that each
iteration of the gadget we get the property that:
\[(P(u),P(u')) = \set{(P(x),0), (0,P(x')), (v,v')} \]
where $v \leq 0.5P(x)$ and $v' \leq 0.5 P(x')$. Repeating the gadget
$m$ times where $2^{-m} \leq 2^{-N}\lambda$ suffices. The property we need
is that we only select one vector or the other -- to ensure this we
simply place ${l \choose 2}$ gadgets: each one says that if $u_i > 0
\implies v_j = 0$ (and vice versa). Observe that the resulting gadget
is polynomial sized. After concatenating the gadgets together the end
result is either a $2^{-N} M_{i_{N}} \cdots M_{i_i}$ (a valid result)
or its $1$ norm is smaller than $\lambda 2^{-N}$ (since it messes up
on at least one of the gadgets).


==> sec_scans.old.tex <==

\subsection{Staccato Approximation Scheme}
We now describe our main technical contribution - the \name approximation scheme to compress an FST.
The key insight here is that the successive strings enumerated by KMAP differ very minimally, as illustrated
in Figure \ref{fig:sc:figure}. This is because successive paths differ usually by just one
edge, since the ranking depends on the overall path probability that is affected by all its edges. This 
prevents the enumeration from bringing in more edges of each transition into the top $K$ paths.

Instead, if we could somehow divide the structure into components, and enumerate top $K$ paths independently over each, 
then, intuitively, we can capture many more strings from the original structure.
This is the key idea behind \name's approximation scheme. 
Instead of storing the full paths (KMAP), we store sets of subpaths, which when concatenated (multiplied) produce
exponentially more strings than KMAP (exponential in the number of such sets), while consuming essentially the same amount of space.
Figure \ref{fig:sc:figure} illustrates this idea.

\begin{figure}[hbtp]
%\textbf{TOP $K$ just wiggles on one character, we break it into
 % blocks. Exponentially better.}
\centering
\includegraphics[width=3.3in]{images/egkmapstaccato}
\caption{Illustration of KMAP vs. \name's approximation. $M$ is the no. of blocks to be produced 
by the \name splitting. Note how the number of strings captured by \name is exponential in $M$.}
\label{fig:sc:figure}
\end{figure}

In the rest of this section, we formalize the notion of splitting an
SFA, show the hardness in achieving it and present our algorithm to
realize the \name approximation.

\subsubsection{SFA Partitioning}
Our goal is to partition an SFA into essentially a union of
SFAs. There are two conceptual steps to our approach to approximate an
SFA: (1) partitioning the nodes into \textit{blocks}, and (2) within
each block, finding the best set of $K$ paths to retain (see
Figure~\ref{fig:sc:figure}). We now describe notations to make these
steps precise.

The input is an SFA $(V,E,s,f,\delta)$. For step (1), we define a {\em
  node-induced edge-partition} (simply, \textit{blocking}) as a set $\Phi
\subseteq 2^{V}$ such that for each $(x,y) \in E$, there is a unique \textit{block}
$\phi \in \Phi$ such that $(x,y) \in \phi$. That is, the defining
property is that every edge is contained in exactly one
partition. Given any $\phi$ denote by $\mathrm{Paths}(\phi)$ the set
of simple paths whose endpoints are contained in $\phi$. For step (2),
given a blocking $\Phi$ an assignment $\alpha$ maps each $\phi$ to a
set of paths (strings) such that $\alpha(\phi) \subseteq
\mathrm{Paths}(\phi)$. We will consider assignments that satisfy the
property that $\size{\alpha(\phi)} \leq K$ for $\phi \in \Phi$. That
is, $\alpha$ selects at most $k$ paths in each block. Given the
original graph, the pair $(\Phi,\alpha)$ defines a probability
distribution $\Pr_{(\Phi,\alpha)}$ in the obvious way.

Our goal to acheive a good approximation is that the distribution
$\Pr_{(\Phi,\alpha)}$ is as close as possible to the
original distribution given by the input SFA, $\Pr_{D}$. We measure
this closeness using the Kullback-Liebler divergence between the
induced distributions:

\[ \KL( \Pr_{(\Phi,\alpha)} || \Pr_D) = \sum_{x \in \mathrm{Paths}(D)} \Pr_{(\Phi,\alpha)}[x] \log \frac{\Pr_{(\Phi,\alpha)}[x]}{\Pr_{D}[x]} \]

%\noindent Our goal is to find $(\Phi,\alpha)$ such that $K$ selects no more than $K$ paths.

We can now state our main hardness result. Essentially, even if we are
given the block structure ($\phi$) the problem is intractable in a strong
sense:

\begin{theorem}
There exists an infinite family of pairs $(D,\Phi)$ where $D$ is an
OCR database and partitions $\Phi$ such that computing $\alpha^{*}$
the following problem is $\mathsf{NP}$-hard in the size of $D$.
\[ \alpha^{*} = \mathrm{argmin}_{\alpha} \KL( \Pr(\Phi,\alpha) || D) \text{ s.t. }
\forall \phi \in \Phi, |\alpha(\phi)| \leq K\]
This remains true even for constant $K$ (explicitly, $K = 52$).
\end{theorem}

The proof essentially reduces non-emptyness of stochastic automata
question to this problem through a gadget construction. A key
technical difficulty is determining the size of alphabet that is
needed, which requires a detailed examination. From this examination,
we are able to show that the hardness ocurrs even for $K$ as small as
$52$.

This strong hardness result motivates us to look for a more tractable approach, leading to our next 
technical contribution - a heuristic restriction on the class of partitions,
which we call the `skinny chains' property. This restriction makes the approximation tractable
and also provides some other desirable properties. Later, we empirically verify that this scheme
is indeed effective and achieves the desired results.


\subsubsection{Skinny Chains Property}
We first define a skinny chain and then discuss more about the importance of this property.\\

\noindent \textbf{Definition:} \textit{A block $\phi$ is a skinny chain iff:}\\
(1) \textit{$\exists ~unique ~node ~\phi_s \in \phi$ (resp. $\phi_e$), which is the minimum 
(resp. maximum) in the partial order on $\phi$, and}\\
(2) $if~ \exists (u,v) \in E ~s.t.~ \phi \cap \{u,v\} \not\subseteq \{\phi_s, \phi_e\}, ~then~ (u,v) \in \phi$\\
% All edges in the original FST that are incident upon any internal nodes of the block (nodes which are neither Min nor Max)
% are present in the block.\\

Basically, a skinny chain is like a miniature SFA on its own. Condition 1 states that a skinny chain has unique start 
and end states. Condition 2 states that a skinny chain has no `portruding edges' in the middle when considered as part 
of the entire partition. Figure \ref{fig:skinnychain} illustrates this concept.

\begin{figure}[hbtp]
[[Figure showing non-skinny vs skinny-chain??.]]
\centering
%\includegraphics[width=3.3in]{images/skinnychain}
\caption{Illustration of skinny chains.}
\label{fig:skinnychain}
\end{figure}


Skinny chains provide an important advantage over general partitions - \textit{sufficient lineage} \cite{approx-lineage}.
Basically, it means that the set of strings produced by $\Phi$ with only skinny chains is a subset of
the set of strings produced by the original SFA. A general partition, however, can wrongly produce strings that are not 
produced by the original SFA \cite{approx-lineage}.

Also, even though we restrict $\Phi$ to skinny chains, this property is general enough to provide another key
desideratum for our approximation scheme - the ability to gracefully tradeoff between KMAP and FullFST. Basically, 
KMAP becomes an extreme case of our approximation, wherein the whole SFA is treated as a skinny chain. 
FullFST, on the other hand, corresponds to the opposite extreme, wherein each transition of the SFA is treated as 
a (miniscule) skinny chain.

As mentioned before, the most important advantage is that the skinny chains property makes the \name 
approximation tractable, unlike the general partition case. Indeed, the computation of the optimal
skinny chain approximation is polynomial in the size of the SFA. This is expressed in the following theorems.

\begin{theorem}
Suppose that $\Phi$ has the skinny chain property, then $\alpha^{*}$
(the minimizer above) can be computed in polynomial time. Moreover,
$\alpha$ selects the $K$ highest paths in each block.
\end{theorem}

[[ Explain ]]
%We can show more:

\begin{theorem}
Let $P$ be the set of all skinny chain partitions for a fixed graph
$G$. Algorithm~\ref{alg:dynamicskinny} finds the optimal partition in time polynomial
in $P$ (cubic) ( -- polynomial in G??)
\end{theorem}

%Combining those theorems gives us that our skinny chain restriction is
%correct. 
%However, cubic is still too expensive in many of our
%applications. Thus, we consider a simple greedy heuristic shown in
%Algorithm~\ref{}.

%Algorithm \ref{alg:dynamicskinny}
%presents a dynamic program that computes the optimal skinny chain partition of a given SFA.\\

[[Explain]]\\

\begin{figure}[hbtp]
[Optimal algorithm?]
\centering
%\includegraphics[width=3.3in]{images/skinnychain}
\caption{Dynamic program-based construction of the optimal \name skinny chain partition.}
\label{alg:greedyskinny}
\end{figure}
 
Thus, we've shown that the skinny chains property provides a practicable approximation scheme. 
However, the runtime of Algorithm \ref{alg:dynamicskinny} is cubic in the size of the SFA, even for a chain SFA (without branching).
Though polynomial, this runtime would likely fare poorly in many of our applications even with modestly large SFAs (few
hundred nodes for an OCR line). Thus, we consider a simple greedy heuristic that is much faster - linear in the size of the SFA.\\ 

[Seems dubious??]\\

\subsubsection{A Fast Greedy Heuristic}
Algorithm \ref{alg:greedyskinny} presents the greedy heuristic for the \name skinny chain partition.
Basically, it starts with the finest partition on the SFA (each transition
as a block) and then iteratively merges blocks to reach the number of blocks specified. It maintains a set of candidate
merges, and at each iteration chooses the best pair to merge. In subsequent iterations, it reuses these candidates to 
avoid recomputation. Note that we need to ensure that the merged blocks satisfy the skinny chain property (the routine 
for this is in the appendix). Also, the `parents' of a new block are the sub-blocks from before the merging that went 
into the new block.

Although the greedy approach may not yield the optimal partition, in practice, we empirically verified
that it yieds good partitions that are able to achieve the high-level goals of our approximation, viz., to provide a knob
to control the recall - performance tradeoff. Later in Section \ref{sec-expts}, we analyze the runtime of this approximation scheme,
and show how the tradeoff plays out on various real-world datasets.

\begin{figure}[hbtp]
\textbf{Inputs:}\\ 
$P$, the base (finest) partition\\
$M$, the no. of blocks parameter\\
$K$, the no. of paths ber block parameter\\
\textbf{Procedure:} $StaccatoConstr(\Pi, M, K)$

\begin{algorithmic}[1]
\STATE Initialize $i \leftarrow  0$ and $P^0 \leftarrow  P$
\STATE Initialize $C^0 \leftarrow  \emptyset$ //candidate merged blocks
\WHILE{$number~ of~ blocks~ in~ P^i > M$}
	\FOR{$each ~adjacent ~block ~pair ~b_p, b_q \in P^i$} 
		\STATE $b_{pq} \leftarrow b_p + b_q$ //graph union
		\IF{$b_{pq} ~is ~not ~a ~skinny ~chain$}
			\STATE $FixCandidate(b_{pq}, P^i)$
		\ENDIF
		\STATE $C^i \leftarrow C^i ~\cup~ \{b_{pq}\}$
	\ENDFOR
%	\STATE //parents of a block are the sub blocks that were merged to obtain it
	\STATE //get the candidate with highest new total probability
	\STATE $c^i_{new} \leftarrow  argmax_{c^i_j \in C^i} TotProb(P^i + c^i_j - c^i_j.parents, K)$ 
%	\STATE //add the new block and remove its parents
	\STATE $\Pi^{i+1} \leftarrow P^i + c^i_{new} - c^i_{new}.parents$
%	\STATE //remove the new block and overlapping candidates
	\STATE $C_{rem} \leftarrow \{c_x ~|~ c_x\in C^i ~and~ \exists c_p \in c_x.parents,~ s.t.~ c_p \cap c^i_{new} ~is ~not ~edgeless\}$
	\STATE $C^{i+1} \leftarrow C^i - c^i_{new} - C_{rem}$
\ENDWHILE
\end{algorithmic}
\caption{Fast greedy heuristic for \name skinny chain partition construction}
\label{alg:greedyskinny}
\end{figure}







%----- old text ------

\begin{comment}

We formalize the approximation as an optimization problem. Treating the FST and the approximate model as a probability 
distribution over strings, we aim to minimize the KL-divergence...

[Explain the mechanics of the approximation]

[Formal problem statement]

[Hardness results/theorems]\\

(Nomenclature - call them `blocks' itself? What about the `blocks' later?)
(Figure to illustrate Staccato on an FST?)\\

Given that the construction of the optimal Staccato approximation is intractable (exponential in the size of the FST), it naturally 
raises the question whether we could construct an efficient heuristic to realize the Staccato idea. This leads us to our next 
technical contribution - a heuristic restriction on the approximate model, which we call the `Skinny Chains' property.

(Why not heuristic approx for non-skinny chains? Logical gap?)

\subsubsection{Skinny Chains Property}

(Explain graph-theoretically or order-theoretically?)

In graph-theoretic terms, an FST can be viewed as a directed graph, with the states being nodes, and transitions being edges. 
In the domains of OCR and speech, the data FSTs do not have cycles, making them DAGs (Directed Acyclic Graphs). They also have 
unique start and end states. Each block in the approximate model (which we henceforth refer to as the `Staccato FST') is thus a 
non-edgeless subgraph of the original FST. We now define the skinny chains property.\\

\noindent Definition: A Skinny Chain is a block that satisfies:\\
(1) Exactly 1 node has in-degree 0 (the `Min')\\
(2) Exactly 1 node has out-degree 0 (the `Max'), and\\
(3) All edges in the original FST that are incident upon any internal nodes of the block (nodes which are neither Min nor Max)
 are present in the block.\\

[Justify skinny chains - sufficiency, lower bound...]
[Mention how it can still cover FullFST to KMAP compression]\\

Henceforth, we use the term Staccato to mean the skinny chain Staccato model.\\

\subsubsection{Staccato Construction}
We now formulate the problem of obtaining the optimal skinny chain Staccato blocks from the original FST as another optimization
problem...

[Formal problem statement for construction]
(Do we need this? Minimizing KL-divergence again?)\\


Unlike the general case, it is possible to optimally solve the skinny chain Staccato approximation 
in polynomial time. Figure \ref{} presents a greedy merge-based algorithm to solve this problem. We start with the base splitting 
of the original FST into per-transition blocks, and then greedily merge blocks to obtain candidate new blocks at each iteration. Before 
propagating new blocks to the next iteration, we ensure the all blocks satisfy the skinny chain property, and if not, we carry out
a fixing operation to obtain larger blocks...

[Describe Staccato Construction Algorithm]
(Present algo here?)

[Optimality results/theorems]

\subsubsection{Query Processing}
(Notation/nomenclature issues?)
We now describe how we handle for handling query procesing over the Staccato data.
A Staccato FST can be viewd as a graph of blocks, wherein each node is a list of K paths. 
Given a regex query, we construct the DFA matrix... 

[Prior art - matrix multiplication approach, cite papers]




\subsection{Analysis}

There are two conceptual parts to our approach to approximate anSFA
(see Figure~\ref{fig:sc:figure}): (1) partitioning the nodes into
blocks, and (2) within each block finding the best set of $k$ paths to
retain. We describe notation to make these steps precise now.


The input is an SFA $(V,E,s,f,\delta)$. For step (1), we define a {\em
  node-induced edge-partition} (simply, blocking) is a set $\Phi
\subseteq 2^{V}$ such that for each $(x,y) \in E$ there is a unique
$\phi \in \Phi$ such that $(x,y) \in \phi$. That is, the defining
property is that every edge is contained in exactly one
partition. Given any $\phi$ denote by $\mathrm{Paths}(\phi)$ the set
of simple paths whose endpoints are contained in $\phi$. For step (2),
given a blocking $\Phi$ an assignment $\alpha$ maps each $\phi$ to a
set of paths (strings) such that $\alpha(\phi) \subseteq
\mathrm{Paths}(\phi)$. We will consider assignments that satisfy the
property that $\size{\alpha(\phi)} \leq k$ for $\phi \in \Phi$. That
is, $\alpha$ selects at most $k$ paths in each block. Given the
original graph, the pair $(\Phi,\alpha)$ defines a probability
distribution $\Pr_{(\Phi,\alpha)}$ in the obvious way.

Our goal to acheive a good approximation is that the distribution
$\Pr_{(\Phi,\alpha)}$ induced by our approximate is close to the
original distribution given by our transducer, $\Pr_{D}$. We measure
this closeness using the Kiellbeck Liebler divergence between the
induced distributions:

\[ \KL( \Pr_{(\Phi,\alpha)} || \Pr_D) = \sum_{x \in \mathrm{Paths}(D)} \Pr_{(\Phi,\alpha)}[x] \log \frac{\Pr_{(\Phi,\alpha)}[x]}{\Pr_{D}[x]} \]

\noindent
Our goal is to find $(\Phi,\alpha)$ such that $k$ selects no more than
$k$ paths.

We can now state our main hardness result. Essentially, even if we are
given the block structure ($\phi$) the problem is intractable in a strong
sense:

\begin{theorem}
There exists an infinite family of pairs $(D,\Phi)$ where $D$ is an
OCR database and partitions $\Phi$ such that computing $\alpha^{*}$
the following problem is $\mathsf{NP}$-hard in the size of $D$.
\[ \alpha^{*} = \mathrm{argmin}_{\alpha} \KL( \Pr(\Phi,\alpha) || D) \text{ s.t. }
\forall \phi \in \Phi, |\alpha(\phi)| \leq k\]
This remains true even for constant $k$ (explicitly, $k = 52$).
\end{theorem}

The proof essentially reduces non-emptyness of stochastic automata
question to this problem through a gadget construction. A key
technical difficulty is determining the size of alphabet that is
needed, which requires a detailed examination. From this examination,
we are able to show that the hardness ocurrs even for $k$ as small as
$52$.

\paragraph*{Positive Results} 
Our first positive result is that if $\Phi$ satisfies the skinny chain
property, then we can simply choose the top $k$ paths in each block.

\begin{theorem}
Suppose that $\Phi$ has the skinny chain property, then $\alpha^{*}$
(the minimizer above) can be computed in polynomial time. Moreover,
$\alpha$ selects the $k$ highest paths in each blcok.
\end{theorem}

[[ Explain ]]

We can show more:

\begin{theorem}
Let $P$ be the set of all skinny chain partitions for a fixed graph
$G$. Algorithm~\ref{alg} find the optimal partition in time polynomial
in $P$ (cubic)
\end{theorem}

Combining those theorems gives us that our skinny chain restriction is
correct. However, cubic is still too expensive in many of our
applications. Thus, we consider a simple greedy heuristic shown in
Algorithm~\ref{alg}.

\end{comment}

